Forgetting-aware Linear Bias for Attentive Knowledge Tracing

Knowledge Tracing (KT) aims to track proficiency based on a question-solving history, allowing us to offer a streamlined curriculum. Recent studies actively utilize attention-based mechanisms to capture the correlation between questions and combine it with the learner's characteristics for responses. However, our empirical study shows that existing attention-based KT models neglect the learner's forgetting behavior, especially as the interaction history becomes longer. This problem arises from the bias that overprioritizes the correlation of questions while inadvertently ignoring the impact of forgetting behavior. This paper proposes a simple-yet-effective solution, namely Forgetting-aware Linear Bias (FoLiBi), to reflect forgetting behavior as a linear bias. Despite its simplicity, FoLiBi is readily equipped with existing attentive KT models by effectively decomposing question correlations with forgetting behavior. FoLiBi plugged with several KT models yields a consistent improvement of up to 2.58% in AUC over state-of-the-art KT models on four benchmark datasets.

==> Previous_writings/sec-abstract.tex <==
\begin{abstract}

% With the rise of online education platforms, there has been a focus on providing learners with a personalized learning experience. 
Knowledge Tracing (KT) aims to track a learner's proficiency based on their problem-solving history, which enables the delivery of a streamlined curriculum. Recently, attention mechanisms have improved KT by effectively modeling the user's interaction with questions. However, no comparative studies have been conducted between methods that address forgetting behavior in attention mechanisms. In this paper, we provide a comparative analysis of different methodologies for forgetting behavior. Furthermore, we propose FoLiBi to adopt the linear bias to attention scores, also known as Attention with Linear Biases (ALiBi), which can effectively consider forgetting behavior in recent attention mechanism-based models called as knowledge retrievers. Despite its simplicity, using it to account for forgetting behavior shows large performance gains over existing forgetting-aware methods. On various benchmark datasets, we validate a consistent performance improvement of x.xx\% to x.xx\% on average for each model by simply adding FoLiBi to the state-of-the-art baselines. We also confirm that as the impact of forgetting behavior increases, i.e., long history, the effectiveness can be further increased.

% In this paper, we propose a method to effectively consider forgetting behavior in recent attention mechanism-based models. The proposed method can be easily adapted to various transformer baselines by adding it as a bias to the attention scores, which is also known as Attention with Linear Biases (ALiBi).
%온라인 학습 플랫폼이 떠오름에 따라 학습자에게 맞춤 학습 경험을 제공하는 것이 큰 관심을 받고 있다. 지식 추적(Knowledge Tracing)이란 학습자의 문제풀이 기록을 바탕으로 학습 성취도를 추적하는 문제로 이를 통해 능률적인 curriculum을 제시할 수 있다. 최근에는 attention mechanism이 질문과 사용자의 interaction을 효과적으로 modeling함으로써 정확도를 향상시켰다. 이 논문을 통해 최근 Attention mechanism 기반 모델에 효과적으로 Forgetting behavior를 고려하는 방법을 제안한다. 제안하는 방법은 Attention score을 계산하는 부분에 추가됨으로써 다양한 transformer baseline에 쉽게 적용될 수 있으며, 기존의 Forgetting-aware methods 대비 안정적인 성능 향상을 보여준다. 다양한 Benchmark 데이터셋에서 기존 baseline 모델에 Alibi만을 추가함으로써 모델 별로 평균 1.14\%~2.58\%의 consistent한 성능 향상을 확인하였으며, forgetting behavior의 영향이 커짐에 따라, i.e., longer history, 제안 방법의 효과가 더욱 커질 수 있음을 확인하였다.





% 본 논문은 어떤 면에서 이와 같은 한계점을 어떻게 극복하려고 하는지 지에 대한 소개
% 	트랜스포머 기반 KT 모델 위에서 attention score에 forgetting behavior를 구현하는 모델별[Basic, RKT, AKT] 비교 실험은 진행된 바 없음. 따라서 기존의 forgetting aware attention mechanism을 비교 분석하고자 함.
% 	본 연구에서는 기존의 고도화된 상대적 위치 임베딩 기법[Rotary, ALiBi]을 도입하여 해결하고자 함. 해당 방법은 query와 key의 내적을 통해 상대적으로 멀리 떨어진 위치의 가중치를 낮게 하고, 가까이 있는 위치의 가중치를 높게 하는 기능이 내재되어 있음으로, 이를 적용하면 자연스럽게 forgetting behavior가 구현될 수 있음. 결과적으로 좀 더 효과적인 ALiBi 방법을 새롭게 도입하여 더 높은 성능 향상을 도출함. 

% 제안 방법의 특징 및 장점 설명
% 	제안 방법은 attention score 계산 시, scalar, non-learned bias값을 추가하여 기존 기록간 유사도 + 상대적 위치에 따른 가중치를 동시에 고려할 수 있음. (해당 방법은 ALiBi를 그대로 사용한 것이기에 이를 변형한 방법제안을 위한 추후 실험이 필요)
% 	Attention 메커니즘에 forgetting을 반영하는 방법 중에서는 제일 우수한 성능을 보임. 
% 	Attention score 시각화를 통해 실제로 제안 방법론과 일치하게 어떤 기록이 강조 되는 지를 설명 가능함. 
% 	본 연구에서는 Forgetting 현상이 문제 풀이 기록의 길이가 길어질수록 심화된다고 봄. 우선, 후반부에 위치한 문제를 기준으로 현재 위치에 가까운 기록을 더 강조하고, 반대의 경우는 덜 강조하는 기능이 필요함. 또한, 문제 풀이 기록의 길이가 길어지더라도 성능을 안정적으로 유지하는 method가 필요함. ALiBi는 이러한 측면에서 기존 방법들 대비 Forgetting 현상을 더 잘 구현하는 강점이 있다고 봄. 



% 지식 추적(Knowledge Tracing)이란 학습자의 문제풀이 기록을 바탕으로 학습 성취도를 추적하는 문제로, 목표 문제가 주어질 때 정답 여부를 예측하는 것을 목표로 한다. 본 연구에서는 ~~ 기존 Transformer 기반 모델들을 비교 모델로 삼아 실험한 결과, 제안 모델인 xx를 적용하였을 때 모든 실험 데이터 셋에서 우수한 성능을 나타냈으며, 기존의 최고 수준 모델 성능 대비 AUC 값이 평균 xx\% 상승하였다. 또한, 대칭적 난이도 표현을 사용하면 순차적 난이도 표현을 사용하는 것보다 AUC 값이 평균 xx\% 더 상승하는 효과를 보였다.
\end{abstract}

\keywords{Knowledge Tracing; Transformer; Forgetting Behavior}

==> Previous_writings/sec-experiments.tex <==
\input{Tables/tab_dataset}
\input{Tables/tab_RQ1}
\input{Figures/fig_RQ2}
\input{Figures/fig_RQ3}

\section{Experiments and Analysis}\label{sec:experiments}
%제안 방법의 효과를 검증하기 위해 다음의 Research Questions에 대한 답변을 하고자 한다.
To verify the effectiveness of our proposed method, we address the following research questions.

\begin{itemize}[leftmargin=5mm]
\item \textbf{RQ1} How does the proposed method perform when used as a plug-in on the state-of-the-art models?
\item \textbf{RQ2} What is the meaningful effect of FoLiBi on attention score in the knowledge retriever? 
\item \textbf{RQ3} Does FoLiBi keep the strength of performance improvements as the input history length varies?
\end{itemize}

\subsection{Experimental Setup}\label{sec:dataset}
\subsubsection{Datasets}\label{sec:dataset}
 %우리는 4가지 real-world 교육 데이터셋을 사용하여 제안 방법의 효과를 평가한다: Algebra 2005-2006 (AL05), Bridge to Algebra 2006-2007 (BR06), ASSISTments 2009-2010 (AS09) \cite{FengHK09AS09}, Slepemapy (SLPY). AL05와 BR06은 KDD컵 2010 EDM 챌린지에서 제공한 대수 학습 이력 데이터셋이다. AS09는 무료 온라인 수학 교육 플랫폼에서 수집한 것으로 지식 추적에 가장 널리 사용된다. SLPY는 온라인 플랫폼 \textit{slepemapy.cz}에서 수집된 지리 학습 이력 데이터셋이다. SLPY 데이터 세트의 경우, 우리는 91,331명의 학습자 중 5,000명의 학습자를 무작위로 샘플링하였다. 가공된 데이터셋의 통계는 표\ref{tab:dataset}에서 확인할 수 있다. 
We evaluate the effectiveness of the proposed method using four real-world education datasets: Algebra 2005-2006 (AL05), Bridge to Algebra 2006-2007 (BR06), ASSISTments 2009-2010 (AS09) \cite{FengHK09AS09}, and Slepemapy (SLPY) \cite{PapousekPS16SLPY}. AL05 and BR06 are algebra learning history datasets provided by KDD Cup 2010 EDM Challenge. AS09 is collected from a free online math education platform and is the most widely used in knowledge tracing. SLPY is a geography learning history dataset collected from the online platform \textit{slepemapy.cz}. Followed by previous work ~\cite{LeeCLPP22CL4KT, Gervet20Preprocess}, we randomly sampled 5,000 learners out of 91,331 learners for the SLPY dataset and performed dataset pre-processing. The statistics of the processed datasets are shown in Table \ref{tab:dataset}. 
\setlength{\parskip}{0.1\baselineskip}
\subsubsection{Baselines and Evaluation}\label{sec:baselines}
%To analyze the effect of different methodologies for forgetting behavior, we use several Transformer-based KT models as backbone models.
To analyze the effect of different methodologies for forgetting behavior, we apply our proposed method to several Transformer-based models. SAKT~\cite{PandeyK19SAKT} is an early model of knowledge tracing using an attention mechanism. AKT~\cite{GhoshHL20AKT} introduces embeddings based on the Rasch model~\cite{Rasch93Rasch} to capture the individual features between different questions and reflect the learner's forgetting phenomenon by formulating an attention mechanism. CL4KT~\cite{LeeCLPP22CL4KT} proposes contrastive learning on the learning histories augmented by proposing four different methods. The Response Prediction Model (RPM) uses the model structure based on AKT and CL4KT. In addition, the question-response pair embedding is expressed as a combination of question embedding and answer embedding as proposed in \cite{GhoshHL20AKT}.
%Forgetting behavior에 대한 여러 방법론의 효과를 분석하기 위해 트랜스포머 기반의 여러 KT 모델을 백본 모델로 사용한다. SAKT\cite{PandeyK19SAKT}는 attention mechanism을 이용한 지식 추적의 초기 모델이다. AKT (Context-Attentive Knowledge Tracing)\cite{GhoshHL20AKT}는 Rasch model\cite{Rasch93Rasch} 기반의 임베딩을 도입하여 문제 사이의 개별적인 특징을 포착하였으며 학습자의 망각 현상을 수식화하여 attention mechanism에 반영한 지식 추적 모델이다. CL4KT (Contrastive Learning for Knowledge Tracing)\cite{LeeCLPP22CL4KT}는 4가지의 문제풀이 기록 증강 방법을 제안하여 증강된 learning histories 간의 대조적 학습을 제안한 지식 추적 모델이다. 본 연구에서 제안하는 RPM (Response Prediction Model)은 AKT와 CL4KT의 기반이 된 모델 구조를 사용하면서 목표 문제에 대한 정답 확률을 예측하기 위해 Binary cross-entropy만을 loss로 정의하여 학습하였다. 또한, 문제-답변 쌍 임베딩을 \cite{0001HL20AKT}에서 제안한 것과 같이 문제 임베딩과 답변 임베딩의 결합으로 표현하였다.
%CL4KT~\cite{LeeCLPP22CL4KT} proposes contrastive learning among the augmented learning histories by proposing four different methods of augmenting each student's learning history.

%우리는 지식 추적의 대표적인 성능 지표인 Area Under Curve(AUC)와 Accuracy(ACC)을 사용한다. AUC, ACC가 1에 가까울수록, RMSE의 값이 0에 가까울수록 모델이 학습자의 답변 예측을 잘 수행한다는 것을 의미한다. 본 연구에서는 데이터의 클래스 불균형을 고려하여 클래스 비율에 따라 예측한 점수에 가중치를 부여하는 Weighted accuracy (w-ACC)를 추가로 확인한다. 클래스 비율이 작을수록 높은 가중치를, 클수록 작은 가중치를 부여한다. Weighted accuracy에 대한 수식은 $\frac{1}{2}\left ( \frac{TP}{TP+FN}+\frac{TN}{TN+FP} \right )$이며, TP, TN, FN, FP는 각각 True-Positive, True-Negative, False-Negative, False-Positive를 의미한다.
%We use Area Under Curve (AUC) and Accuracy (ACC), which are typical performance metrics for knowledge tracing. The closer the AUC and ACC are to 1, and the closer the value of RMSE is to 0, the better the model performs in predicting learners' answers. In this study, we further examine Weighted accuracy (w-ACC), which takes into account the class imbalance in the data and weights the predicted scores according to the class proportions. The smaller the class ratio, the higher the weight, and the larger the class ratio, the lower the weight. The formula for weighted accuracy is $\frac{1}{2}\left ( \frac{TP}{TP+FN}+\frac{TN}{TN+FP} \right )$, where TP, TN, FN, and FP stand for True-Positive, True-Negative, False-Negative, and False-Positive, respectively. 
We use Area Under Curve (AUC) and Accuracy (ACC), which are typical metrics for knowledge tracing. In this study, we further examine weighted accuracy (w-ACC), which takes into account the class imbalance by weighting the class proportions. The formula is as follows: $\frac{1}{2}\left ( \frac{TP}{TP+FN}+\frac{TN}{TN+FP} \right )$, where TP, TN, FN, and FP stand for True-Positive, True-Negative, False-Negative, and False-Positive, respectively. 
\setlength{\parskip}{0.1\baselineskip} 
\subsubsection{Implementation Details}\label{sec:details}
%데이터 전처리는 가장 최근의 기록만을 추출하는 방식을 따르며, 하나의 문제에 대하여 다수의 개념(concept)이 대응되는 경우, 고유한 개념 조합의 개수를 기준으로 개념 고유번호를 부여하였다 \cite{Gervet20Preprocess}. 학습자별 문제-답변 쌍의 최소 개수는 5로 제한하였다. 
%We followed recent research to preprocess dataset~\cite{Gervet20Preprocess}. The minimum number of question-response pairs per learner was limited to 5.
%We consider the most recent histories, and in cases where multiple concepts correspond to a single question, we assign a unique number based on the number of unique concept combinations \cite{Gervet20Preprocess}.
%데이터 셋은 5-fold 교차 검증을 적용하여 5개의 fold에 대한 평균값을 실험 결과로 사용하였다. Test fold를 제외한 나머지 fold에 대하여 90\%를 Train 데이터 셋으로, 10\%를 Validation 데이터 셋으로 나누었다. 
%We perform 5-fold cross-validation and use the average of the five folds as the final result. For the remaining folds, except for the test fold, we divided 90\% into the training dataset and 10\% into the Validation dataset.
We perform 5-fold cross-validation on 3 different seeds and report the average.
%모든 모델 학습에 Adam optimizer가 사용되었으며, 학습률(learning rate)은 0.001, 배치 크기(batch size)는 512으로 설정하였다. 최대 300번의 에폭(epoch)을 반복하여 학습하면서 Validation 데이터 셋에 대하여 AUC가 10 에폭 동안 증가하지 않으면 학습을 조기 중단한다. 
We use Adam optimizer with a learning rate of 0.001, and a batch size of 512. We iteratively train for up to 300 epochs and stop training if the AUC does not increase for 10 epochs on the validation dataset. 
%베이스라인의 임베딩 크기는 64, 어텐션 헤드(head) 수는 8개, 어텐션 블록(block) 수는 2개로 고정하였다. 나머지 하이퍼파라미터5는 Optuna\cite{AkibaSYOK19OPTUNA}를 통해 데이터별로 최적화된 값을 바탕으로 비교 모델 및 제안 모델 결과를 기재하였다.
%We fixed the embedding size to 64, the number of attention heads to 8, and the number of attention blocks to 2 for all models. The remaining hyperparameters were optimized for each dataset using Optuna \cite{AkibaSYOK19OPTUNA}, and the results of the comparison model and the proposed model are shown.
We fixed the embedding size to 64, the number of attention heads to 8, and the number of attention blocks to 2 for all models. The remaining hyperparameters were optimized for each dataset using Optuna~\cite{AkibaSYOK19OPTUNA}. We set the history length to 100 for all experiments except the one where we varied the inference length (Figure \ref{fig:fig_RQ3}); for that experiment, we set the maximum length to 300 and varied the maximum number of interactions to input.
%All the source code will be released upon acceptance.

==> Previous_writings/sec-introduction.tex <==
\section{Introduction}\label{sec:introduction}


% 현재 작성된 서론에서 첫 번째 문장이 주제문으로 보기가 어려워 보이는데,
%확인 후 주제문을 수정하여 그에 맞게 단락을 구성해 보기 바랍니다.

% 지식 추적에 대한 소개 및 중요성
% 기존에 지식 추적 연구에 대한 설명 및 주요 특징
% 지식 추적 연구에서 가장 중요한 부분이 (1) 문제 간 상관 관계 분석과 (2) 망각 효과에 대한 구현을 대표적인 두 가지 특징으로 해석할 수 있을까요?
% 최근 망각 효과에 대한 연구 설명 및 한계점
% 제안 방법에 대한 소개 및 장점
% 본 논문에 대한 요약


% 위 주제문을 바탕으로 다음과 같이 재구성해보았습니다. 

% 지식 추적에 대한 소개 및 기존 모델들의 주요 특징(문제 간 상관 관계 분석)
% 망각 효과를 고려하는 지식 추적 모델들을 transformer 기반 모델인지 여부로 분류 
% 망각 효과를 고려하는 transformer 변형 모델들의 주요 특징 및 한계점
% 제안 방법에 대한 소개 및 장점
% 본 논문에 대한 요약


온라인 교육 시스템의 대중화에 따라 누적되는 방대한 양의 학습 기록을 바탕으로, 지식 추적은 지능형 교육 서비스를 개발하기에 앞서 학습자의 지식 상태를 관찰하고, 표현하고, 정량화하는 task이다. 구체적으로 학습자에게 새로운 문제가 주어졌을 때, 학습자의 과거 문제 풀이 기록으로부터 구체화되는 지식 숙련도를 파악하여 해당 문제를 맞힐 확률을 정확하게 예측하는 것을 목표로 한다. 최근에는 다양한 관점에서 딥러닝 기반을 모델을 이용하여 지식 추적 문제를 해결하고 있으며, 그 중에는 learning curve theory\cite{Ebbinghaus2013forgetcurve}을 고려하여 예측 정확도를 고도화하려는 모델들\cite{NagataniZSCCO19DFKT, ShenLCHHYS021LPKT, Abdel2021DGMN, ChenLHWCWSH17KPT, ShinSYLKC21SAINT+, PandeyS20RKT, GhoshHL20AKT}이 제안되어 왔다. 

이들은 학습자가 아주 오래 전에 쌓인 기록을 잊는 망각 현상이 학습자의 지식 상태에 큰 영향을 미치는 요소임~\cite{Pavlik2005INTRO, Pelanek15aINTRO2, Sense2016INTRO3}을 고려하여, 이러한 복잡한 현상을 모델 내에서 단순화하여 구현하고자 하였다. 대표적으로 목표 문제와 이전 기록 간의 time interval에 대한 정보를 모델의 입력으로써 제공해주는 구현 방법이 있다. DFKT~\cite{NagataniZSCCO19DFKT}와 LPKT~\cite{ShenLCHHYS021LPKT}는 LSTM 기반의 DKT~\cite{PiechBHGSGS15DKT}를 backbone 모델로 하면서 forget effect를 고려하기 위해 풀이 기록 간 time interval 정보를 입력에 반영하였다. HawkesKT~\cite{WangMZLWLT0M21HawkesKT}는 matrix factorization 기반 KT 모델~\cite{VieK19KTM}을 개선하기 위해 concept간 유사도와 time interval 정보를 결합하여 concept에 따라 망각 정도가 다를 수 있다는 temporal cross-effect를 구현하고자 하였다.

한편, Several works~\cite{ShinSYLKC21SAINT+, GhoshHL20AKT, PandeyS20RKT}는 문제 풀이 기록 간의 long-term dependencies를 효과적으로 capture하기 위해 self-attention module을 사용함과 동시에 학습자의 문제별 숙련도를 학습자의 기억 능력과 연관지어 파악하고자 하였다. SAINT+~\cite{ShinSYLKC21SAINT+}는 트랜스포머 기반의 KT 모델~\cite{PandeyK19SAKT} 계열 중 하나로, 수집된 real-time 데이터를 바탕으로 서로 다른 concept을 가진 풀이 기록 간의 time interval을 입력에 반영하였다. 이와 다르게 \cite{GhoshHL20AKT, PandeyS20RKT}는 attention mechanism 내에서 forgetting effect를 효과적으로 구현하는 방법론을 제안하였다. Attention score에 query와 key 간의 time interval bias를 더해줌으로써 거리가 상대적으로 먼 위치에 놓인 기록에 덜 집중하는 효과를 가지도록 하였다. 

그러나, 본 연구에서는 기존 방법론들이 여전히 time interval이 긴 상황에서 time interval 정보를 온전히 고려하기 어렵다고 판단한다. 따라서, 이러한 forgetting-aware attention mechanism들의 효과를 먼저 비교 분석하고, 그 다음 기존의 고도화된 상대적 위치 임베딩 기법인 ALiBi\cite{PressSL22ALiBi}을 도입함으로써 결과적으로 입력 시퀀스 길이에 상관없이 효과적으로 forgetting behavior를 수행할 수 있는 방법 FoLiBi을 제안하였다. 
We summarize our contributions as follows. 
\begin{itemize}[leftmargin=5mm]
\item 기존에 제안되었던 forgetting-aware attention mechanism 기법들을 다른 트랜스포머 기반 모델들에 적용하여 효과를 비교하였다.
\item 제안 방법인 FoLiBi가 기존 SOTA KT 모델의 AUC 성능을 significantly 향상시킬 수 있음을 Real-world 교육 데이터셋에 대한 extensive experiments로 검증하였다.   
\item 제안 방법은 다른 방법론들 대비 다양한 길이의 입력에도 견고한 성능을 보이는 효과를 가지는 것을 확인하였다.  
\end{itemize}




==> Previous_writings/sec-method.tex <==
\input{Figures/fig_1.tex}

% \section{Modeling Forgetting Behavior}\label{sec:method}
\section{Proposed Method}\label{sec:method}

\subsection{Problem Definition}\label{sec:definition}
% \vspace{1mm}
% \noindent
% \textbf{Problem Definition.}
Knowledge tracing (KT) is commonly formulated as a sequential response prediction problem for each question. Let $X_{t-1} = \langle x_1, x_2 ..., x_{t-1}\rangle$ denote a sequence of observed interactions for questions at the $(t-1)$-th time step. Each interaction $x_i=(q_i,r_i)$ consists of a pair of a question $q_i$ and its correctness $r_i\in [0,1]$. Here, $r_i=1$ means that $q_i$ is answered correctly and $r_i$=1 means that $q_i$ is answered incorrectly. Given a sequence of interactions $X_{t-1}$, KT models aim to predict the probability of correctly answering the question $q_t$ at the $t$-th time step, \ie, $\hat{r}_t= p(r_t = 1 \mid X_{t-1}, q_t)$. For the loss function, they commonly adopt a binary cross-entropy function used in the classification problem.

% $E=\{e_1, e_2, ..., e_{|E|}\}$ denote a set of exercises in a datset and 

%문제풀이 기록의 최대 길이인 $T$의 각 시점 $t$에서 $q$는 문제이고, $r$은 학습자의 정오답 정보를 나타낸다. 학습자가 문제를 틀린 경우 $r=0$이고, 그렇지 않으면 $r=1$이다. 즉, 다음과 같이 $X_{u}=\langle x_1, ..., x_{t-1}\rangle$가 주어질 때, 바로 다음 시점의 목표 문제 $q_t$에 대한 정답 여부 $r_t$가 1인 확률 $\hat{r_t}$을 계산한다. 
% \begin{equation}
% \hat{r_t}=p(r_t=1 | x_1, x_2, ..., x_{t-1}, q_t).
% \end{equation}

% 기존 지식 추적 모델의 입력 임베딩 방식\cite{PiechBHGSGS15DKT, PandeyK19SAKT, ZhangSKY17DKVMN, LeeCLPP22CL4KT}을 따르면 문제 $q$와 답변 $r$에 대하여 각각 문제 임베딩 $e\in R^{C\times d}$과 문제-답변 쌍 임베딩 $i\in R^{2C\times d}$을 정의할 수 있다. 여기서 $C$는 고유한 개념(concept)의 개수이고 $d$는 임베딩 벡터 차원의 크기를 의미한다. 

\subsection{Attentive Knowledge Tracing Model}\label{sec:ExistingKT}
% \vspace{1mm}
% \noindent
% \textbf{Existing KT models with the attention mechanism.}
Recent KT models, \eg, SAKT~\cite{PandeyK19SAKT}, SAINT~\cite{ChoiLCBKCSBH20SAINT}, AKT~\cite{GhoshHL20AKT}, RKT~\cite{PandeyS20RKT}, and CL4KT~\cite{LeeCLPP22CL4KT}, primarily utilize a transformer architecture using a self-attention mechanism to compute $\hat{r}_t$. Compared to conventional RNN models, the attention mechanism helps us better learn hidden patterns across questions/responses, even if interaction sequences are long. Figure \ref{fig:fig1} depicts the architecture of KT models using the self-attention block. To fully capture the correlation between questions, recent models decompose two parts, computing the attention weights $\boldsymbol{\alpha_t}\in\mathbb{R}^{1 \times (t-1)}$ of questions and aggregating responses. First, two encoders represent hidden vectors for questions and responses. Then, the self-attention block calculates the question correlations as attention weights and aggregate responses as a linear combination of attention weights.
\begin{equation}
\boldsymbol{\alpha}_t=\operatorname{softmax}\left(\frac{\mathbf{q}_t \mathbf{K}^{\top}}{\sqrt{d}} \right), \mathbf{v}_t = \boldsymbol{\alpha}_t \mathbf{V} 
\end{equation}
where $d$ is the dimension size of key, query, and value embedding vectors. Let $\mathbf{q}_t \in \mathbb{R}^{1 \times d}$, $\mathbf{K} \in \mathbb{R}^{(t-1) \times d}$, and $\mathbf{V} \in \mathbb{R}^{(t-1) \times d}$ denote the query vector for target question $q_t$, the key matrix for previous questions $(1\leq i <t)$, and the value matrix for previous responses, respectively. Despite its simplicity, it benefits from preventing unnecessary intervention between questions and responses. 

%Query and key vectors are derived from questions to calculate the attention weight between previous questions $(1\leq\tau<t)$ and a target question $q_t$. Then, the values for responses are aggregated to predict the answer to the target question. 



\subsection{Modeling Forgetting Behavior}

In this work, we further investigate forgetting behavior used in the attention mechanism. Forgetting behavior represents a failure in the user’s learning memory or skill proficiency, depending on the temporal distance. The further in the past, the less important the correlation between the previous question and the target question, \emph{i.e.}, the user’s memories gradually decay over time. It is vital to understand users’ latent learning process over time. Several studies~\cite{} have incorporated forgetting behavior into the attention block. We formulate the forgetting behavior used in the attention mechanism, \emph{i.e.}, AKT~\cite{GhoshHL20AKT} and RKT~\cite{PandeyS20RKT}.
\begin{equation}
\label{eq:general_attention}
\boldsymbol{\alpha}_t=\operatorname{softmax}(\frac{\mathbf{q}_t \mathbf{K}^{\mathrm{T}}+\boldsymbol{\beta}_t}{\sqrt{d}}) + \boldsymbol{\gamma}_t,
% \begin{gathered}
% \alpha_{t, \tau}=\frac{\exp (s_{t, \tau})}{\sum_{\tau^{\prime}} \exp (s_{t, \tau^{\prime}})} + \beta_{t,\tau}, \ s_{t, \tau} = \frac{q_t k_\tau^\top + \gamma_{t,\tau}}{\sqrt{D_k}},
% \end{gathered}
\end{equation}
where $\boldsymbol{\beta}_{t} \in \mathbb{R}^{t-1}$ and $\boldsymbol{\gamma}_{t} \in \mathbb{R}^{t-1}$ are additional coefficients to represent forgetting behavior according to $t$-th time step. 

%The correlation between the previous questions and target question is less critical
%Forgetting behavior in knowledge tracing is based on the notion\cite{MozerPCLV09MCM, Ebbinghaus2013forgetcurve} that learning is temporal and learners' memories gradually decay. Previous work using self-attention blocks has modeled forgetting behavior together with attention weights $\alpha$. They can be generally expressed as,
%지식 추적에서 forgetting behavior는 학습은 일시적이고(temporal) 학습자의 기억은 점차 상실(decay)된다는 점\cite{MozerPCLV09MCM, Ebbinghaus2013forgetcurve}에 기반한다. 기존 Attentive encoder를 활용하는 Knowledge tracing 연구들은 attention weights $\alpha$에 forgetting behavior를 함께 모델링한다. They can be generally expressed as,


% where $D_k$는 key embedding의 dimension을 나타내며, $q_t$는 query embedding of $t$-th exercise를, $k_\tau (\tau<t)$는 key embedding of $\tau$-th exercise를 나타낸다. $\beta$와 $\gamma$는 each method에서 서로 다르게 forgetting behavior를 모델링 하기 위해 사용하는 term이다.

AKT~\cite{GhoshHL20AKT} uses a \emph{monotonic attention (Mono)}, which incorporates forgetting behavior into the attention weight. Although it considers temporal decay for previous questions, it heavily affects the correlation between questions and the target question. It indicates that AKT~\cite{GhoshHL20AKT} does not fully decompose forgetting behavior from question correlations.
% Monotonic attention (Mono)\cite{GhoshHL20AKT}은 $\beta$를 활용하여 Softmax function 이전의 logit에 forgetting behavior를 address.
\begin{equation}
\boldsymbol{\beta}_{t}^{\text {Mono }}=(\exp(-\theta_h \cdot \mathbf{d}_{t}-1) \cdot \mathbf{q}_{t} \bold{K}^{\top}, \ \gamma_{t}^{\text {Mono }}=\vec{0},
% \beta_{t, \t}^{\text {Mono }}=0, \ \gamma_{t, \tau}^{\text {Mono }}=(\exp(-\theta_h \cdot d_{t}-1) \cdot q_{t} k_\tau^{\top},
\end{equation}
% \beta^{monotonic}_i = (\exp({-\theta \cdot d(i,\tau)}) - 1)\cdot q_iK^\top, \\
% \gamma^{monotonic}_i = 0.
where, $\mathbf{d}_{t}=\{d(\tau, t), \tau \in [1, \dots, t-1]\}$ consists of the relative distance between $\tau$-th question and a target question multiplied by the cumulative similarity. $\theta_h$ is a learnable decay rate parameter for the $h$-th head in the multi-head attention block.

% $\theta_h>0$는 a learnable decay rate parameter for $h$-th head이다. $d(\tau, t)$는 $\tau+1 $부터 $t-1$시점 까지의 exercise들의 key embeddings와 $q_t$의 cumulative 유사도에 $t$와 $\tau$의 distance, \ie, $t-\tau$, 를 곱해줌으로써 거리에 따른 penalty를 부여한다. 


Then, RKT~\cite{PandeyS20RKT} devises a \emph{relational coefficient (RC)} that combines the question similarity and forgetting behavior. Although RC accounts for the temporal correlations for forgetting behavior, it is also limited in effectively decoupling forgetting behavior from question correlations.
% \cite{PandeyS20RKT}는 Equation \ref{eq:general_attention}의 $\gamma$를 통해 기존의 scaled dot-product attention weight에 relation coefficients(RC)를 추가한다.
\begin{equation}
\boldsymbol{\beta}_{t}^{\text {RC }}=\vec{0}, \ \boldsymbol{\gamma}_{t}^{\text {RC }}=\operatorname{softmax}(\mathbf{R}^E+\mathbf{R}^T),
% \beta_{t, \tau}^{\text {RC }}=\frac{\exp (R^E_\tau+R^t_\tau)}{\sum_{\tau^{\prime}} \exp (R^E_{\tau^{\prime}}+R^t_{\tau^{\prime}})}, \ \gamma_{t, \tau}^{\text {RC }}=0.
\end{equation}
where $\mathbf{R}^E$ represents the relational similarities between previous questions and the target question, and $\mathbf{R}^T=\{\exp{(-(t-\tau)/S)}, \tau \in [1, 2, \dots, t-1]\}$ consists of the relative time interval normalized by a learnable decay rate S. For simplicity, we omit a linear combination of $\boldsymbol{\alpha}_t$ and $\boldsymbol{\gamma}_t$, in RKT~\cite{PandeyS20RKT}.

% $X$의 exercise로 이루어진 $E=\langle e_1, e_2 ..., e_{t-1}\rangle$에 대해 $R^E_\tau\in \mathbb{R}^1$는 $e_\tau$와 $e_t$의 유사도를 나타내며 $R^t_\tau$ is defined as $\exp(-(t-\tau) / S)$ denoting relative time interval between $t$ and $\tau$. Here, $S \in \mathbb{R}^1$는 trainable parameter로 learner의 memory를 나타낸다. Note that we omitted $\lambda$ used for weighted averaging in the original paper. For a more detailed explanation of both methods, see \cite{GhoshHL20AKT, PandeyS20RKT}.

% \begin{equation}
% \mathbf{R}^t=\langle \exp(-(t-1) / S_u), \exp(-(t-2) / S_u), \ldots, \exp(-1 / S_u) \rangle.
% \end{equation}
\vspace{1mm}
\noindent

In this paper, we introduce a simple yet effective method, namely \emph{forgetting-aware linear bias (FoLiBi)}, to effectively integrate the question correlation with forgetting behavior. The key design principles of our proposed method are two-fold. (i) It should decouple question correlations and forgetting behavior. (ii) It should temporally decay question correlations to reflect forgetting behavior. Note that forgetting behavior may affect various factors such as problem difficulty and user personality, but we mainly consider it as temporal relationships for questions. Inspired by recent work~\cite{PressSL22ALiBi} that designs a linear bias for relative position distance, we represent forgetting behavior as a linear bias over time.
\begin{equation}
\boldsymbol{\beta}_{t}^{\text {FoLiBi}}=m_h\cdot [1, \dots, t-1], \ \boldsymbol{\gamma}_{t}^{\text {FoLiBi}}=\vec{0},
\end{equation}
where $m_h$ represents different coefficients for the $h$-th head in multi-head attention, indicating different forgetting behavior across attention heads.

Figure \ref{fig:fig_RQ2} visualizes the different attention weights between existing models and ours. Existing models mostly consider question correlations similar to conventional position embedding (PE). Despite its simplicity, FoLiBi effectively penalizes temporal decay for forgetting behavior. Because it is also independent of computing the question correlations, FoLiBi effectively decomposes two key factors in computing attention weights. As a result, it penalizes the correlation for long-interval questions and emphasizes the correlation for shot-interval questions. In Table~\ref{}, experimental results show that our simple-yet-effective method plugged into several KT models consistently outperforms existing KT models up to XX\% performance gains on several benchmark datasets.




%기존의 방법론들은 모두 궁극적으로 두 가지 직관을 반영한다: $i$) 목표 문제와 관련된 문제이면서 $ii$) 상대적으로 가까이 위치한 문제에 대하여 더 집중하도록 설계한다. 그러나 both approaches는 forgetting behavior를 modeling하는 term, \ie, $\beta$ and $\gamma$,에 exercise간의 유사도가 함께 계산됨으로써 순서 정보를 온전히 반영하지 못한다. 특히 figure X와 같이 $X$의 길이가 길어짐에 따라 유사도에 의존적인 attention map을 보여주는 결과로 이어진다. Thanks to the recent work by \cite{PressSL22ALiBi}, 우리는 두 가지 직관을 분리하고 간결하게 하는 FoLiBi을 제안한다. From the equation \ref{eq:general_attention}, 제안하는 forgetting behavior의 modeling term은 다음으로 정의된다.

% where $m_h$ is a slope for the $h$-th head based on a pre-defined geometric sequence. $H$를 head의 숫자라고 할 때, $m_h$는 $2^{\frac{-8}{H}\cdot h}$로 계산된다. $\mathbf{\gamma}^{\text {FoLiBi}}_t$는 \cite{PressSL22ALiBi}에서 소개하는 bias와 같으며 \cite{GhoshHL20AKT, PandeyS20RKT}과 달리 exercise간의 유사도로부터 독립적인 modeling을 수행한다. 이로써 FoLiBi는 간단하지만 명확하게 두 가지 직관을 동시에 구현한다.% 하는 방법론이다.


\iffalse
본 연구에서는 forgetting mechanism을 구현하기 위해 기존 scaled dot-product 집중 메커니즘에 다음의 두 가지 직관을 반영하고자 한다: $i$) 목표 문제와 가장 관련된 문제이면서 $ii$) 상대적으로 가까운 위치에 놓인 문제에 대하여 더 집중하도록 설계한다. 길이 $T(1 \leq i \leq T)$인 문제풀이 기록에 대한 attention score을 계산할 때, $i$번째 query인 $q_i \in \mathbb{R}^{1 \times d}$와 keys $K_i \in \mathbb{R}^{i \times d}$에 decay bias term $b=[0, 1, 2, \ldots, i-1]$을 더하여 다음과 같이 표현한다.: 
\begin{equation}
\alpha_i = softmax(q_iK^\top + m \cdot b),
\end{equation}
여기서 $d$는 head의 dimension을 나타낸다. scalar $m$은 head의 수 $H(1 \leq j \leq H)$에 따라 정해지는 geometric sequence $2^{-8/H}+2^{-8/H}(j-1)$를 사용하여 사전 정의된 head-specific slope이다. $b$는 linearly constant bias로, query와 key 사이의 내적값에 인접한 위치에 대해 높은 가중치를 부여하여 결과적으로 서로 유사한 문제들 중에서도 가까운 위치에 놓인 문제에 더 집중시키는 기능을 한다. Note that we don't use positional embeddings when using linear bias.
%attention score 계산 시 $m \cdot b$ term을 사용할 때는 KT모델에 위치 임베딩을 더하지 않는다.    
\fi


% Knowledge retriever의 목표는 배치 내 모든 학습자들에 대하여 목표 값인 $r_t$와 예측값 $\hat{r_t}$사이의 binary cross-entropy를 줄이는 것이다.
% \begin{equation}
% \mathcal{L} = -\sum_{\tau=2}^{t}{r_\tau log \hat{r_\tau} + (1-r_\tau) log(1-\hat{r_\tau})} \\ \\
% \mathcal{L} = -r_t \log(\hat{r_t}) - (1-r_t) \log(1-\hat{r_t})
% \end{equation}

% 대표적으로 \cite{GhoshHL20AKT, LeeCLPP22CL4KT}의 경우, 집중 메커니즘 기반의 문제 인코더 $g^E$, 문제-답변 쌍 인코더 $g^I$를 이용하여 문제 임베딩 $e_{1:t}\in \mathbb{R}^{C\times d}$과 문제-답변 쌍 임베딩 $i_{1:t-1}\in \mathbb{R}^{2C\times d}$을 각각 $h^E_{1:t}$, $h^I_{1:t-1}$이라는 맥락-인식(context-aware) 임베딩으로 변환하는 중간 과정을 거친다. 여기서 $C$는 고유한 개념(concept)의 개수이고 $d$는 임베딩 벡터 차원의 크기를 의미한다. 그 다음 $h^E_{t}$, $h^E_{1:t-1}$, $h^I_{1:t-1}$이 각각 query, key, value가 되어 Knowledge Retriever $f^{KR}$을 통과하면 $v_t$를 얻는다. $m_c$는 집중 모듈 내에서 후속 위치의 집중 가중치를 0으로 만들어 미래의 정보를 제외하는 집중 마스크이다.:
% \begin{equation}
% v_t=f^{KR}(query = h^E_{t}, key = h^E_{1:t-1}, value = h^I_{1:t-1} ; m_c),
% \end{equation}

==> Previous_writings/sec-results.tex <==
% \subsection{Overall Performance (RQ1)}\label{sec:rq1}
\subsection{Results and Analysis}\label{sec:results}

% 1. FoLiBi의 AUC가 모든 setting에서 best
% 2. backbone 모델, dataset에 따라 Monotonic attention과 RC 방법론은 서로 

Table \ref{tab:performance} shows the performance of different forgetting behavior modeling methods using different backbone models on the four benchmark datasets. While Positional Embedding (PE) incorporates absolute location information into the input embedding, Monotonic attention (Mono), Relational Coefficient (RC), and FoLiBi design the coefficients $\boldsymbol{\beta}$ and $\boldsymbol{\gamma}$ differently to reflect temporal decay. The key observations are as follows: (1) Mono and RC perform better than PE by accounting for relative distance, but in most cases, there is no significant performance difference between them. This is because both approaches include a correlation between questions when considering forgetting behavior. However, all backbone models show the highest AUC performance across all datasets when FoLiBi is plugged in. It confirms that FoLiBi is the most appropriate method to commonly trace learners' knowledge by avoiding the intervention between two objectives, \ie, question and temporal correlation. (ii) Applying FoLiBi to CL4KT~\cite{LeeCLPP22CL4KT} shows a relatively small improvement over Mono, with a 1.1\% improvement, but RPM with the same model structure and removing contrastive loss increases the performance improvement to 1.5\%. It implies that contrastive learning in CL4KT~\cite{LeeCLPP22CL4KT} makes the model more dependent on question correlations, suggesting that it is important to balance question and temporal correlation. (iii) The difference between ACC and w-ACC shows a prediction bias toward the correct answer class, \ie, 1, which has a high proportion of the class. FoLiBi significantly improves the baseline models in the w-ACC metric, indicating that FoLiBi also helps to mitigate the prediction bias of KT models.


%PE는 절대적인 위치 정보를 KT 모델의 입력 임베딩에 반영하는 방법이다. Mono, RC, FoLiBi는 temporal dacay를 고려하는 coefficients $\boldsymbol{\beta}_t$과 $\boldsymbol{\gamma}_t$를 각각 달리 설계한 방법이다. The key observations are as follow: (1) Monotonic attention과 RC 방법론은 relative distance를 고려함으로써 PE보다는 좋은 성능을 보이지만 대다수의 경우 큰 성능 차이를 보이지 않는다. 이는 두 방법론 모두 forgetting behavior를 고려할 때 문항간의 correlation을 포함하는 방식을 따르기 때문이다. However, all backbone models show the highest AUC performance across all datasets when FoLiBi is plugged in. It confirms that FoLiBi is the most appropriate method to commonly account for question correlation and forgetting behavior by preventing the intervention between two objectives, \ie, question and temporal correlation. (ii) FoLiBi를 CL4KT에 적용하는 경우 monotonic attention 보다 1.1\% 개선하여 상대적으로 적은 향상폭을 보였으나, 동일한 모델 구조를 갖고 contrastive loss를 제거한 RPM은 1.5\%로 성능 개선이 증가한다. 이는 CL4KT의 대조 학습으로 인해 모델이 문항 간의 corrleation에 더욱 dependent한 모델이 되었기 때문으로, question correlation과 temporal correlation을 균형있게 고려하는 것이 중요하다는 것을 의미한다. (iii) ACC와 w-ACC의 차이는 클래스 비율이 높은 정답 클래스, \ie, 1, 에 대한 예측 편향성이 나타나는 것을 암시한다. FoLiBi는 w-ACC 지표에서도 baseline 모델들을 significantly 개선하여 FoLiBi가 KT 모델의 예측 편향성을 완화하는 데에도 도움이 되었다는 것을 보여준다.

%본 연구에서는 표 \ref{tab:dataset} 처럼 클래스가 불균형한 것을 고려하여 클래스별로 weight를 다루게 주어 평가하는 weighted accuracy(w-ACC) metric을 도입한다. 
% 표 \ref{tab:performance}는 풀이 기록의 길이가 100인 데이터셋을 기준으로 모든 모델들에 대한 AUC, ACC, w-ACC 평가 결과를 보여준다. Baselines 위에서 Position Encoding(PE), Monotonic Attention(Mono), RC(Relational Coefficient), 그리고 FoLiBi를 각각 적용하여 성능을 비교했다. Position Embedding(PE)는 순차적 위치 정보를 KT 모델의 입력 임베딩에 반영하는 방법이다. Mono, RC, FoLiBi는 temporal dacay를 고려하는 coefficients $\boldsymbol{\beta}_t$ 또는 $\boldsymbol{\gamma}_t$를 각각 달리 설계한 방법이다. FoLiBi의 경우, 모든 데이터 및 baseline 모델들에 적용했을 때 AUC를 기준으로 가장 높은 성능을 보여 그 효과를 검증했다. 즉, 제안 방법이 plug-in으로써 기존의 knowledge retriever 형태의 KT 모델들의 성능을 신장시키는 효과가 있는 것을 확인하였다. OO는 모든 데이터셋에 대하여 AUC가 평균 X.XX\%p가 상승하며 가장 높은 성능 개선을 보였다. 그 다음으로 AKT가 평균 X.XX\%p 상승하여 AKT가 제안한 monotonic attention보다 FoLiBi를 통한 forgetting behavior를 더 효과적으로 모델링한다는 것을 확인할 수 있다. CL4KT의 경우 평균 X.XX\%p로 다른 베이스라인 모델들과 비교하여 가장 낮은 성능 개선을 보였으나, CL4KT 동일한 모델 구조를 갖고 contrastive loss를 제거한 RPM이 X.XX\%p의 상승을 보이는 것으로 보아, 


% 상대적 위치 부호화 방법인 Rotary와 FoLiBi를 각각 적용하였을 때, SAKT의 경우에는 Rotary와 FoLiBi 둘 다 모든 데이터에 대해 monotonic attention보다 AUC 성능이 개선되었음을 확인할 수 있다. 또한, 모든 데이터와 베이스라인에 대해 Rotary보다 FoLiBi가 ACC 기준 우수한 성능을 보였다.

% 본 연구에서는 표 \ref{tab:dataset}에서 확인한 것처럼 데이터별 클래스 분포가 불균형한 것을 고려하여 weighted accuracy(w-ACC)를 도입하여 모델 성능을 종합적으로 비교하였다. 기존 KT 모델들이 ACC 대비 w-ACC에 대하여 모두 낮은 값을 가지는 것으로 보아, 상대적으로 클래스 비율이 높은 클래스 1에 대한 예측 편향성이 나타나는 것으로 해석된다. w-ACC 지표에서도 다른 평가 지표 대비 성능이 매우 큰 폭으로 증가하며 개선된 것을 보여 FoLiBi가 KT 모델의 예측 편향성을 완화하는 데에도 도움이 되었다고 본다.


%표 \ref{tab:performance}는 풀이 기록의 길이가 100인 데이터 셋을 기준으로 모든 baseline 모델들에 대한 AUC, ACC, w-ACC 평가 결과를 보여준다. FoLiBi의 경우, AUC를 기준으로 모든 데이터 및 baseline 모델들에 적용했을 때 가장 높은 성능을 보여 그 효과를 검증했다. 즉, 제안 방법이 plug-in으로써 기존의 knowledge retriever 형태의 KT 모델들의 성능을 신장시키는 효과가 있는 것을 확인하였다. SAKT는 모든 데이터에 대하여 AUC가 평균 7.58\%p가 상승하여 가장 높은 성능 개선을 보였다. 그 다음으로는 AKT가 평균적으로 6.24\%p 상승하여 AKT가 제안한 monotonic attention보다 제안 방법이 대체로 더유용하다는 것을 확인할 수 있었다. CL4KT의 경우, 3.45\%p로 다른 baseline 모델들과 비교했을 때 가장 낮은 개선을 보였으나, 동일한 모델 구조를 가지는 RPM이 4.66\%p만큼 개선된 것으로 보아 RPM에서 contrastive loss를 제거한 것과 새로운 문제-답변 쌍 임베딩 방법을 도입한 것이 FoLiBi 적용에 도움이 된 것으로 판단된다.    

%표 \ref{tab:performance}는 풀이 기록의 길이가 100인 데이터 셋을 기준으로 모든 baseline 모델들에 대한 AUC, ACC, w-ACC 평가 결과를 보여준다. 베이스라인에 상대적 위치 부호화 방법인 Rotary, FoLiBi를 적용함으로써 성능을 비교하였다. 기존 SAKT에서는 forgetting behavior를 적용하지 않았으며 AKT, CL4KT, 그리고 RPM에서는 monotonic attention가 적용된다. FoLiBi의 경우, 모든 데이터 및 baseline 모델들에 적용했을 때 AUC 기준 가장 높은 성능을 보임을 확인할 수 있다. 즉, FoLiBi를 통한 forgetting behavior modeling이 plug-in으로써 기존의 knowledge retriever 형태의 KT 모델들 성능을 신장시키는 효과가 있음을 검증하였다. SAKT는 모든 데이터에 대하여 AUC가 평균 7.58\%p가 상승하여 가장 높은 성능 개선을 보였다. 그 다음으로는 AKT가 평균적으로 6.24\%p 상승하여 AKT가 제안한 forgetting behavior인 monotonic attention을 FoLiBi로 대체하였을 경우, 제안 방법이 효과적으로 forgetting behavior를 표현할 수 있음을 보인다. CL4KT의 경우, 3.45\%p로 다른 baseline에 비해 비교적 가장 낮은 개선을 보였으나, 동일한 모델 구조에 contrastive loss를 제거한 RPM이 4.66\%p만큼 개선되었다. Contrastive learning을 통해 문제의 잠재 개념 유사도를 학습하기보다 FoLiBi를 통한 forgetting behavior 적용과 새로운 문제-답변 쌍 임베딩 방법을 도입하는 것이 학습 상태를 모델링하는 데에 더 적절하다고 판단할 수 있다.

% \subsection{Visualizing Forgetting Mechanism (RQ2)}\label{sec:rq2}
% PE 대비 MONO, RC, FoLiBi 모두 대각선만을 강조하는 것이 아니라, 이전 문제들 중에 연관도가 높은 문제들에 대해서도 강조하는 모습을 보임. 
% FoLiBi는 후반부의 위치에 대해서도 문제의 유사도와는 독립적으로 가까운 위치에 대한 강조를 잘하는 모습을 보임. 
\vspace{1mm}
\noindent
\textbf{Comparison via attention weights.}
Figure \ref{fig:fig_RQ2} visualizes the attention weights of the first 20 questions for the first head in the last self-attention block of the knowledge retriever in RPM. We randomly sampled two learners from AL05 and the x and y axes of each map represent the previous question and the target question, respectively. Thus, it is possible to understand how relevant past histories are relative to the current one. While Mono, RC, and FoLiBi all give higher scores to questions that are close to the target, we found that FoLiBi considers the relative position distance information more, and this tendency holds especially for long sequences (>10). This is because Mono and RC are more affected by question correlation as well as temporal decay when computing $\boldsymbol{\beta}_t$ and $\boldsymbol{\gamma}_t$, respectively, as the relative distance difference increases. On the other hand, FoLiBi uses a static, non-learned $\boldsymbol{\beta}_t$, which means that a temporal relation can have a constant influence on the attention score regardless of the learning outcome.  As a result, FoLiBi is a more effective implementation of the forgetting mechanism than the other methods in this study.
% 1) This is likely due to the fact that Mono and RC rely more on question correlation than temporal decay as the relative distance difference increases to calculate $\boldsymbol{\beta}_t$ and $\boldsymbol{\gamma}_t$, respectively.
%Figure \ref{fig:fig_RQ2} visualizes the attention weights of the first 20 questions for the first head in the last self-attention block of the knowledge retriever in RPM. We randomly sampled two learners from AL05 dataset and the x and y axes of the each map represent the previous question and the target question, respectively. 따라서 현재 시점의 기록을 기준으로 과거 기록들이 얼만큼 관련이 있는지 이해할 수 있다. 상대적인 위치 거리 정보를 고려하는 Mono, Rc, and FoLiBi가 모두 target문제와 가까운 문제에 높은 점수를 주지만, FoLiBi가 더 많이 고려하고 있으며, 특히 이러한 경향을 특히 긴 sequence(>10)에 대해서도 유지하는 것을 확인하였다. 이는 Mono, RC가 각각 $\boldsymbol{\beta}_t$, $\boldsymbol{\gamma}_t$를 계산함에 있어서 상대적인 거리 차가 커질수록 temporal decay보다 question correlation에 더 의존하기 때문인 것으로 판단된다. 반면에 FoLiBi는 static, non-learned $\boldsymbol{\beta}_t$을 사용하기 때문에 학습 결과에 상관없이 termporal relation의 일정한 영향력을 attention score에 미칠 수 있다. 결과적으로 본 연구에서 도입한 FoLiBi가 다른 방법 대비 forgetting mechanism을 더 효과적으로 구현한 방법이라고 볼 수 있다.

% Figure \ref{fig:fig_RQ2}은 knowledge retriever의 마지막 self-attention block 내 첫번째 head에 대한 attention score을 forgetting behavior 모델별로 시각화한 것이다. 문제 풀이 기록의 길이가 100일 때 AUC 성능이 가장 높은 RPM 모델의 AL05 데이터에서 학습자 두 명을 랜덤하게 샘플링하여 분석 대상으로 삼았다. Map의 x축과 y축은 각각 과거 위치 인덱스와 현재 위치 인덱스를 의미한다. 따라서 현재 시점의 기록을 기준으로 과거 기록들이 얼만큼 관련이 있는지 이해할 수 있다. 먼저 PE는 문제의 유사도만을 고려하여 attention score을 계산하기 때문에 현재 시점의 문제를 기준으로 먼 위치에 놓인 문제에 대해서도 강조하는 부분을 확인할 수 있다. 한편, Mono, RC와 FoLiBi의 경우, 문제의 유사도뿐만 아니라 현재 시점의 기록을 기준으로 가까이 위치한 과거 기록일수록 더 강조하여 보는 경향이 있다. 세 가지 방법 모두 additional coefficients $\boldsymbol{\beta}_t$ 또는 $\boldsymbol{\gamma}_t$을 이용하여 학습자의 forgetting behavior를 구현한 점이 반영되었다고 본다. 한편, FoLiBi가 Mono, RC에 비해 후반부에 위치하는 기록, 즉, 대각선에 대해서 진한 색을 보이는 것으로 보아, 길이가 긴 sequence에 대해서도 forgetting behavior가 더 잘 보존된 것을 확인할 수 있다. 이는 Mono, RC가 각각 $\boldsymbol{\beta}_t$, $\boldsymbol{\gamma}_t$를 계산함에 있어서 상대적인 거리 차가 커질수록 temporal decay보다 question correlation에 더 의존하기 때문인 것으로 판단된다. 반면에 FoLiBi는 static, non-learned $\boldsymbol{\beta}_t$을 사용하기 때문에 학습 결과에 상관없이 termporal relation의 일정한 영향력을 attention score에 미칠 수 있다. 결과적으로 본 연구에서 도입한 FoLiBi가 다른 방법 대비 forgetting mechanism을 더 효과적으로 구현한 방법이라고 볼 수 있다.  



% 전반적으로 길이가 50까지 길어질수록 성능이 급격히 증가하다가, 그 이상부터는 완만하게 증가함. 길이가 길수록 학습자의 학습과정을 더 많이 반영하여 예측 성능을 높이는 데 도움이 됨. 
% PE 대비 나머지 모델들의 꺾은 선이 더 상위에 위치함. 즉, forgetting behavior고려하는 것이 좋음
% RC와 Mono 비교
% folibi는 길이가 100보다 짧거나 길어도 강건한 성능을 유지함. 
\vspace{1mm}
\noindent
\textbf{Strength on varying history length.}
In this section, we conducted additional experiments to see if the proposed method retains its effectiveness on data with varying lengths of the problem-solving history. Figure \ref{fig:fig_RQ3} shows the AUC of the RPM model for four different data sets. The model was trained on data of length 300 and compared to the same test set with increasing lengths of 10, 20, 50, 100, 200, and 300. The lines of RC, Mono, and FoLiBi are higher than that of PE, indicating that the forgetting-aware attention mechanism is an important operation in the KT task. In addition, FoLiBi outperformed the second-best performing methodology for each dataset by a significant margin. For the shortest lengths of 10, FoLiBi outperforms the second best model by 2.04\%, 1.18\%, 0.81\%, and 0.05\% for AL05, BR06, AS09, and SLPY, respectively. For the longest length of 300, FoLiBi's performance surpassed the second-best model by 2.92\%, 2.00\%, 0.77\%, and 1.73\%, respectively. While SLPY has a small performance difference of 0.05\% with the second-best model, RC, for length 10, RC's performance decreases as input sequence length surpasses 100, whereas FoLiBi shows a consistent improvement.


% \subsection{Strength on Varying History Length (RQ3)}\label{sec:rq3}
% 본 연구에서는 제안 방법이 입력 시퀀스의 길이가 100보다 짧거나 긴 데이터에 대해서도 효과적인 성능을 보이는지 알아보기 위해 추가적인 실험을 진행하였다. 그림 \ref{fig:fig_RQ3}는 네 가지의 데이터별로 문제 풀이 기록의 길이에 따라 변화하는 RPM 모델의 AUC를 나타낸 것이다. 모델은 길이 300인 데이터로 학습하였으며, 같은 test 셋에 대하여 평가 대상의 길이를 10, 20, 50, 100, 200 그리고 300까지 늘려가며 비교하였다. 모든 경우에 대하여 history의 길이를 길게 학습할수록 성능이 높아지는 경향이 있다. 특히 길이가 50까지 길어질수록 성능이 급격히 향상되며 그 이상일수록 완만하게 성능이 증가하였다. 전반적으로 문제 풀이 기록의 길이가 길수록 학습자의 학습 과정을 더 많이 반영하여 KT 모델의 예측 성능을 높이는 데 도움이 된다는 것을 알 수 있다. 또한, PE 대비 RC, Mono, FoLiBi 모델의 꺾은선이 더 상위에 위치하는 것으로 보아 Forgetting mechanism이 KT task에 중요하게 반영되어야 할 요소라고 할 수 있다. RC는 Mono와 비교했을 때 AS09, BR06 데이터와 SLPY의 50 이하 길이 데이터에서 조금 더 우수하였다. 한편, FoLiBi는 모든 데이터셋과 길이에 대해 다른 방법론들과 비교하여 가장 높은 성능을 보이는 것을 확인할 수 있다. 길이가 10일 경우, FoLiBi는 각 데이터셋에 대해 두 번째로 높은 성능을 보이는 방법론과 비교하여 AL05, BR06, AS09, 그리고 SLPY 각각 1.57\%p, 0.89\%p, 0.59\%p, 그리고 0.03\%p 더 높은 성능을 보였고, 길이가 가장 긴 300에 대해서는 2.30\%p, 1.57\%p, 0.58\%p, 그리고 1.27\%p의 성능 차이를 보이며 FoLiBi가 긴 시퀀스에 대해 강점을 보임을 증명하였다. 특히 SLPY의 경우, 길이 10에서 성능이 두 번째로 높은 RC와 0.03\%p의 근소한 차이를 보였지만, 길이가 100이상 길어질수록 RC는 성능이 감소하는 경향을 보이는 반면, FoLiBi는 완만하더라도 꾸준히 증가하는 모습을 보였다. 입력 시퀀스의 길이가 길어져도 강력한 성능을 유지하는 장점을 가질 뿐만 아니라, 길이가 짧은 경우에 대해서도 기존 모델들 대비 우수한 성능을 보였다.

\iffalse
\subsection{Strength on Varying History Length (RQ3)}\label{sec:rq3}
본 연구에서는 제안 방법이 입력 시퀀스의 길이가 100보다 짧거나 긴 데이터에 대해서도 효과적인 성능을 보이는지 알아보기 위해 추가적인 실험을 진행하였다. 그림 \ref{fig:fig_RQ3}는 네 가지의 데이터별로 문제 풀이 기록의 길이에 따라 변화하는 RPM 모델의 AUC를 나타낸 것이다. 모델은 길이 300인 데이터로 학습하였으며, 같은 test 셋에 대하여 평가 대상의 길이를 10, 20, 50, 100, 200 그리고 300까지 늘려가며 비교하였다. 모든 경우에 대하여 History의 길이를 길게 학습할수록 성능이 높아지는 경향이 있다. 특히 길이가 50까지 길어질수록 성능이 급격히 향상되며 그 이상일수록 완만하게 성능이 증가하였다. 전반적으로 문제 풀이 기록의 길이가 길수록 학습자의 학습 과정을 더 많이 반영하여 KT 모델의 예측 성능을 높이는 데 도움이 된다는 것을 알 수 있다. 또한, PE 대비 RC, Mono, FoLiBi 모델의 꺾은선이 더 상위에 위치하는 것으로 보아 Forgetting mechanism이 KT task에 중요하게 반영되어야 할 요소라고 할 수 있다. RC는 Mono와 비교했을 때 AS09, BR06 데이터와 SLPY의 50 이하 길이 데이터에서 조금 더 우수하였다. 한편, FoLiBi는 입력 시퀀스의 길이가 길어져도 강력한 성능을 유지하는 장점을 가질 뿐만 아니라, 길이가 짧은 경우에 대해서도 기존 모델들 대비 우수한 성능을 보였다.
\fi

